BiPMAP: A Toolbox for Predictions of Perceived Motion Artifacts on Modern Displays

Presenting dynamic scenes without incurring motion artifacts visible to observers requires sustained effort from the display industry. A tool that predicts motion artifacts and simulates artifact elimination through optimizing the display configuration is highly desired to guide the design and manufacture of modern displays. Despite the popular demands, there is no such tool available in the market. In this study, we deliver an interactive toolkit, Binocular Perceived Motion Artifact Predictor (BiPMAP), as an executable file with GPU acceleration. BiPMAP accounts for an extensive collection of user-defined parameters and directly visualizes a variety of motion artifacts by presenting the perceived continuous and sampled moving stimuli side-by-side. For accurate artifact predictions, BiPMAP utilizes a novel model of the human contrast sensitivity function to effectively imitate the frequency modulation of the human visual system. In addition, BiPMAP is capable of deriving various in-plane motion artifacts for 2D displays and depth distortion in 3D stereoscopic displays.

==> Text/acknowledgments.tex <==
\section{Acknowledgments}

==> Text/introduction.tex <==
\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
\IEEEPARstart{M}{odern} displays constitute an interface bridging the two ends of an information delivery system: the electronic signal delivered to the display, and the human observers receiving the information converted to light by the interface. For effective communication and pleasant visual experiences, the interface needs to be optimized in order to fit the capabilities of human visual systems. Therefore, display manufacturers have spent tremendous effort to optimize the design of their display products, e.g., monitors, projectors, virtual-reality (VR) and augmented reality (AR) headsets, etc., and one of the main routes leads to the appropriate representation of dynamic scenes. Although the motion of an object in a dynamic scene is always presented through a discrete sequence of static views, a proper design of the display device will ensure human observers see an object moving smoothly across the display. In contrast, given an improper display configuration,motion artifacts will be perceived instead. \par
A variety of motion artifacts need to be contemplated when designing a display device. Flickering, which is perceived discontinuity in  

% \subsection{Subsection Heading Here}
% Subsection text here.

% % needed in second column of first page if using \IEEEpubid
% %\IEEEpubidadjcol

% \subsubsection{Subsubsection Heading Here}
% Subsubsection text here.

==> Text/methods.tex <==
\section{Methods}

Methods text here.

\subsection{Input parameters}

\subsection{Display parameters}

\subsection{Human vision model}

\subsection{Viewing parameters}





==> Text/results.tex <==
\section{Results}

==> backup/conclusion.tex <==
\section{Conclusion}
